Quantification of Differential Information using Matrix Pencil

Any traditional classification problem in general involves modelling individual classes and in turn classification by evaluating the similarity of the test set with the modelled classes. In this paper, we introduce another approach that would find the differential information between two classes rather than modelling individual classes separately. The classes are viewed on a common frame of reference in which one class would have a constant variance, unlike the other class which would have unequal variance along its basis vectors which would capture the differential information of one class over the other.This, when mathematically formulated, leads to the solution of Matrix Pencil equation.The theory of binary classification was extended to a multi-class scenario.This is borne out by illustrative examples on the classification of the MNIST database.

==> notsubmitted.tex <==
\section{Generation of Transformation Independent Basis for deterministic signals}
\par KL basis has been explored hugely for a wide set of applications in case of the stochastic signals.  The motivation of this work is to find patterns invariant to a class of transformations applied on all kinds of deterministic signal.  
The theory presented so far has been derived for stochastic signals we can extend the same for the case of finite length deterministic signals.  Let us consider a set $\ddot{s}$ of finitely many transformation such that $\ddot{s} \triangleq \{\tau_{1}, \tau_{2}.  .  .  .  .  .  , \tau_{n}\}$.  This class would encompass all types of transformations such as translation, rotation, scaling such that the transformed object lies in a finite window.Without loss of generality we can assume that the mean of the signal is equal to zero so orthogonality and uncorrelatedness can be used interchangeably. Let a signal X be represented in terms of orthogonal basis $\{{\phi_{k},  1 \leq k \leq n}\}$.  Let $\tau $ be any action applied on X which would form the transformed version of signal X denoted as $\tau.  X$ which can be expressed in terms of the same basis vectors $\{{\phi_{k},  1 \leq k \leq n}\}$ . Here $a_{k}(\tau)$ are coefficients regarded as a function of transformations. The set of transformations is a finite set hence $a_{k}(\tau)$ would be a vector in the finite dimensional space. We assume that there are N such transformations hence $a_{k}(\tau)$ would lie in the N dimensional vector space for each $k$.  Regarding this $a_{k}(\tau)$ to lie in the N dimensional space we intend to find $\{{\varphi_{k},  1 \leq k \leq n}\}$ such that the coefficients $a_{k}(\tau)'s$ are orthogonal. Let us denote identity transformation on the signal $X$ as $I.X$ and its corresponding projection coefficients as $a_{k}(I)$.
\newline
\begin{equation}
\label{equation 35}
\begin{split}
I.X &= \sum\limits_{k} a_k(I)\varphi_k \\
\tau .   X &= \sum\limits_{k} a_k(\tau) \varphi_k \\
a_k(\tau) &=  \langle \tau .   X , \varphi_k\rangle 
\end{split}   
\end{equation}
$a_k(\tau)$ represents the value of projection coefficients as a function of the transformation $\tau$.  Let us at this point define a vector $a_{k}$ such that 
$a_{k}(\tau) = [a_{k}(\tau_{1})\,\ a_{k}(\tau_{2})\,\ .  .  .  .  .  .  .  .  .  a_{k}(\tau_{n})]$ which is the value of $k^{th}$ projection coefficient for the entire set of transformation $\tau$.  The projection coefficients are a function of the transformation on the signal and can be regarded as a mapping from the transformation set $\ddot{s}$ $\mapsto$ $\mathbf{R}$.  
\begin{theorem}
Let X be a deterministic signal and $\tau .   X$ be any transformation such that $X = \sum\limits_{k} a_k\varphi_k$ then $ a_{k}(\tau)$ and $ a_{l}(\tau) $ are orthogonal if and only if $\varphi_k$ are solution to the eigen value problem.  
\end{theorem} 
\begin{proof}
In order to prove that $a_{k}(\tau) $ and $ a_{l}(\tau)$ are orthogonal the below stated equation has to be satisfied.  

\begin{equation}
\label{equation 36}
\langle a_{k}(\cdot) , a_{l}(\cdot)\rangle = \delta_{k, l}\lambda_{k}  
\end{equation}

\begin{equation}
\label{equation 37}
\begin{split}
&\sum\limits_{\tau_{p}} a_{k}(\tau_{p})a_{l}^*(\tau_{p}) \\
&=  \sum\limits_{\tau_{p}}  \sum\limits_{i} X(\tau_{p}(i))\varphi_{k}(i)\sum\limits_{j} X^*(\tau_{p}(j))\varphi_{l}^*(j) \\
&=\sum\limits_{\tau_{p}}[\sum\limits_{i}(\tau_{p} .   X)(i)\varphi_{k}(i)][\sum\limits_{j}(\tau_{p} .X)^{*}(j)\varphi_{l}^{*}(j)] \\
&=\sum\limits_{i}\sum\limits_{j}[\sum\limits_{\tau_{p}}(\tau_{p} .X)(i)(\tau_{p}.   X)^*(j)]\varphi_{k}(i)\varphi_{l}^*(j) \\
&=\sum\limits_{i}\sum\limits_{j}R_{xx}(i, j)\varphi_{k}(i)\varphi_{l}^{*}(j) \\
\end{split}
\end{equation}
If $a_{k}(\tau) $ and $ a_{l}(\tau)$ are orthogonal then using equation \ref{equation 36} we have:
\begin{equation}
\label{equation 38}
   \sum\limits_{i}\sum\limits_{j}R_{xx}(i, j)\varphi_{k}(i)\varphi_{l}^{*}(j) = \delta_{k, l}\lambda_{k} 
\end{equation}
Which can be true if and only if equation \ref{equation 39} is satisfied.
\begin{equation}
\label{equation 39}
\sum\limits_{j}R_{xx}(i, j)\varphi_{k}(i) = \lambda_{k} \varphi_{k}(i)
\end{equation}
Considering $\Re$ to be an operator such that $\Re = R_{xx}(i, j) $.The above equation in operator form can also be written as:
\begin{equation}
    \label{equation 40}
    \Re \phi = \lambda \phi
\end{equation}
Thus it can be clearly stated that the orthogonality of $a_{k}(\tau) $ and $ a_{l}(\tau)$ can only be established when $\,\ \{{\phi_{k},  1 \leq k \leq n}\}$ is the solution to the standard eigen value problem.
Simplifying equation \ref{equation 38} using equation \ref{equation 37} we can obtain the following:
\begin{equation}
\label{equation 41}
\begin{split}
\sum\limits_{\tau_{p}} a_{i, k}(\tau_{p})a_{j, l}^{*}(\tau_{p}) &= \sum\limits_{i}\lambda_{k} \varphi_{k}(i)\varphi_{l}^{*}(i) \\
\sum\limits_{\tau_{p}} a_{i, k}(\tau_{p})a_{j, l}^{*}(\tau_{p}) &= \delta_{k, l} \lambda_{k}
\end{split}
\end{equation}
\end{proof}
\subsection {Discussion}
The above theory was tested for various types of deterministic signals.The correlation matrix of the deterministic is computed using equation \ref{equation 37}. It was observed that for any deterministic signal and its transformed versions the correlation of various projection across the set of transformations was an approximate identity matrix.  Except for an ill- conditioned matrix when the ratio of the maximum and minimum eigen value of the correlation matrix was $\gg 100$ the projection coefficients are not completely uncorrelated. In such cases when the correlation matrix was ill-conditioned the eigen values which constituted $95\% $ of the energy were selected. The orthogonality of the coefficients across the various translations is in conjunction with the fact that the coefficients carry independent information when the basis were a solution to the eigen value problem.Since the coefficients considered as a function of the transformation are orthogonal this framework would be quite useful in identification of pattern which are invariant to the class of transformations.
